LLM-based Query Expansion Fails for Unfamiliar and Ambiguous Queries

Query expansion (QE) enhances retrieval by incorporating relevant terms, with large language models (LLMs) offering an effective alternative to traditional rule-based and statistical methods. However, LLM-based QE suffers from a fundamental limitation: it often fails to generate relevant knowledge, degrading search performance. Prior studies have focused on hallucination, yet its underlying cause--LLM knowledge deficiencies--remains underexplored. This paper systematically examines two failure cases in LLM-based QE: (1) when the LLM lacks query knowledge, leading to incorrect expansions, and (2) when the query is ambiguous, causing biased refinements that narrow search coverage. We conduct controlled experiments across multiple datasets, evaluating the effects of knowledge and query ambiguity on retrieval performance using sparse and dense retrieval models. Our results reveal that LLM-based QE can significantly degrade the retrieval effectiveness when knowledge in the LLM is insufficient or query ambiguity is high. We introduce a framework for evaluating QE under these conditions, providing insights into the limitations of LLM-based retrieval augmentation.

==> tables/rq1_table.tex <==
\begin{tabular}{lllcccccccc}
\hline
                                                 &                                             &                           & \multicolumn{2}{c}{NQ}                                                                     & \multicolumn{2}{c}{TQA}                                                                    & \multicolumn{2}{c}{MS MARCO}                                                               & \multicolumn{2}{c}{BioASQ}                                            \\ \cline{4-11} 
Retrieval                                        & LLM                                         & Expansion                 & NDCG@10                           & Recall@100                                             & NDCG@10                           & Recall@100                                             & NDCG@10                           & Recall@100                                             & NDCG@10                           & Recall@100                        \\ \hline
\multicolumn{1}{l|}{\multirow{6}{*}{BM25}}       & \multicolumn{1}{l|}{\multirow{3}{*}{GPT}}   & \multicolumn{1}{l|}{Q2E}  & \cellcolor[HTML]{FEF3F3}0.25      & \multicolumn{1}{c|}{\cellcolor[HTML]{F1F1FC}-0.55}     & \cellcolor[HTML]{FEF7F7}0.14      & \multicolumn{1}{c|}{\cellcolor[HTML]{FEFBFB}0.05}      & \cellcolor[HTML]{FEB7B5}\bf{3.46} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD9693}\bf{5.89}} & \cellcolor[HTML]{FEE1E0}0.96      & \cellcolor[HTML]{FDAFAD}\bf{3.99} \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Q2D}  & \cellcolor[HTML]{FEB5B3}\bf{3.55} & \multicolumn{1}{c|}{\cellcolor[HTML]{FED6D5}\bf{1.53}} & \cellcolor[HTML]{FEDAD9}\bf{1.30} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEEBEA}0.55}      & \cellcolor[HTML]{FD9895}\bf{5.75} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD7F7C}\bf{7.81}} & \cellcolor[HTML]{EDEDFB}-0.80     & \cellcolor[HTML]{FEC6C4}2.47      \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{GaQR} & \cellcolor[HTML]{FEE6E6}0.73      & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFE}-0.05}     & \cellcolor[HTML]{FEEAEA}0.56      & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF2F2}0.27}      & \cellcolor[HTML]{FED2D1}\bf{1.74} & \multicolumn{1}{c|}{\cellcolor[HTML]{FED1D0}\bf{1.81}} & \cellcolor[HTML]{E2E3FA}-1.53     & \cellcolor[HTML]{FEDCDB}1.20      \\ \cline{2-11} 
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{\multirow{12}{*}{L-8b}} & \multicolumn{1}{l|}{Q2E}  & \cellcolor[HTML]{FED2D1}\bf{1.76} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF4F3}0.23}      & \cellcolor[HTML]{FEE8E8}\bf{0.64} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEE7E6}\bf{0.71}} & \cellcolor[HTML]{FEBBB9}\bf{3.19} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD9F9C}\bf{5.22}} & \cellcolor[HTML]{E7E7FA}-1.18     & \cellcolor[HTML]{FEB8B6}3.35      \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Q2D}  & \cellcolor[HTML]{FECDCC}\bf{2.02} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEE2E1}0.94}      & \cellcolor[HTML]{FEE6E5}\bf{0.75} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEEEED}0.44}      & \cellcolor[HTML]{FDA09D}\bf{5.13} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD8F8C}\bf{6.49}} & \cellcolor[HTML]{F2F3FC}-0.46     & \cellcolor[HTML]{FEE7E6}0.71      \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{GaQR} & \cellcolor[HTML]{FEFCFC}0.03      & \multicolumn{1}{c|}{\cellcolor[HTML]{EEEFFC}-0.69}     & \cellcolor[HTML]{FEFCFC}0.03      & \multicolumn{1}{c|}{\cellcolor[HTML]{FEEFEE}\bf{0.40}} & \cellcolor[HTML]{FED1D0}\bf{1.78} & \multicolumn{1}{c|}{\cellcolor[HTML]{FECDCC}\bf{2.04}} & \cellcolor[HTML]{E3E4FA}-1.44     & \cellcolor[HTML]{FED2D1}1.73      \\ \cline{1-1} \cline{3-11} 
\multicolumn{1}{l|}{\multirow{3}{*}{ANCE}}       & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Q2E}  & \cellcolor[HTML]{FEDFDE}1.06      & \multicolumn{1}{c|}{\cellcolor[HTML]{FED4D3}\bf{1.62}} & \cellcolor[HTML]{FEDEDE}\bf{1.09} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEE5E4}\bf{0.81}} & \cellcolor[HTML]{FEC4C2}\bf{2.59} & \multicolumn{1}{c|}{\cellcolor[HTML]{FDB1AE}\bf{3.89}} & \cellcolor[HTML]{F2F2FC}-0.49     & \cellcolor[HTML]{F1F1FC}-0.53     \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Q2D}  & \cellcolor[HTML]{FEBAB8}\bf{3.24} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEB5B3}\bf{3.56}} & \cellcolor[HTML]{FDB1AF}\bf{3.86} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEC4C3}\bf{2.57}} & \cellcolor[HTML]{FEB7B6}\bf{3.41} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD9592}\bf{6.03}} & \cellcolor[HTML]{ECECFB}-0.83     & \cellcolor[HTML]{FDA7A4}4.62      \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{GaQR} & \cellcolor[HTML]{FEDBDA}\bf{1.27} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEEAEA}0.56}      & \cellcolor[HTML]{FEDFDE}\bf{1.07} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEE2E1}\bf{0.94}} & \cellcolor[HTML]{FEBDBC}\bf{3.01} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEB4B2}\bf{3.67}} & \cellcolor[HTML]{FEDDDC}1.16      & \cellcolor[HTML]{FD9C99}\bf{5.43} \\ \cline{1-1} \cline{3-11} 
\multicolumn{1}{l|}{\multirow{3}{*}{Contriever}} & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Q2E}  & \cellcolor[HTML]{FEC0BE}\bf{2.84} & \multicolumn{1}{c|}{\cellcolor[HTML]{FED2D1}\bf{1.74}} & \cellcolor[HTML]{F7F8FD}-0.21     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF0F0}0.35}      & \cellcolor[HTML]{FDACA9}\bf{4.25} & \multicolumn{1}{c|}{\cellcolor[HTML]{FDAAA8}\bf{4.35}} & \cellcolor[HTML]{FD8B88}\bf{6.83} & \cellcolor[HTML]{FD706D}\bf{9.17} \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Q2D}  & \cellcolor[HTML]{FDA3A1}\bf{4.86} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEB5B3}\bf{3.60}} & \cellcolor[HTML]{FEC9C8}\bf{2.26} & \multicolumn{1}{c|}{\cellcolor[HTML]{FED5D4}\bf{1.57}} & \cellcolor[HTML]{FD9794}\bf{5.86} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD8E8B}\bf{6.55}} & \cellcolor[HTML]{FD7C78}\bf{8.13} & \cellcolor[HTML]{FD6E6A}\bf{9.38} \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{GaQR} & \cellcolor[HTML]{FED4D3}\bf{1.61} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEDFDE}\bf{1.07}} & \cellcolor[HTML]{FEE0DF}\bf{1.03} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEE0E0}\bf{1.00}} & \cellcolor[HTML]{FDB3B1}\bf{3.74} & \multicolumn{1}{c|}{\cellcolor[HTML]{FDA7A4}\bf{4.60}} & \cellcolor[HTML]{FD9E9C}\bf{5.27} & \cellcolor[HTML]{FD837F}\bf{7.53} \\ \cline{1-1} \cline{3-11} 
\multicolumn{1}{l|}{\multirow{3}{*}{E5-base-v2}} & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Q2E}  & \cellcolor[HTML]{FEB5B3}\bf{3.55} & \multicolumn{1}{c|}{\cellcolor[HTML]{FDABA9}\bf{4.29}} & \cellcolor[HTML]{EAEAFB}-1.00     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEECEB}0.51}      & \cellcolor[HTML]{FDA9A7}\bf{4.45} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD7E7B}\bf{7.90}} & \cellcolor[HTML]{FDA19F}\bf{5.02} & \cellcolor[HTML]{FD7C78}\bf{8.13} \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Q2D}  & \cellcolor[HTML]{FEC2C0}\bf{2.71} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEB4B2}\bf{3.63}} & \cellcolor[HTML]{FEE6E5}0.74      & \multicolumn{1}{c|}{\cellcolor[HTML]{FED8D7}\bf{1.42}} & \cellcolor[HTML]{FD928F}\bf{6.25} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD726E}\bf{9.03}} & \cellcolor[HTML]{FD8986}\bf{6.98} & \cellcolor[HTML]{FD706C}\bf{9.22} \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{GaQR} & \cellcolor[HTML]{F6F6FD}-0.27     & \multicolumn{1}{c|}{\cellcolor[HTML]{FECBC9}\bf{2.18}} & \cellcolor[HTML]{F0F0FC}-0.59     & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF5F5}0.18}      & \cellcolor[HTML]{FED4D2}\bf{1.66} & \multicolumn{1}{c|}{\cellcolor[HTML]{FDA5A3}\bf{4.73}} & \cellcolor[HTML]{FD9895}\bf{5.76} & \cellcolor[HTML]{FDA29F}\bf{4.97} \\ \hline
\end{tabular}

==> tables/rq2_query_expansion_methods.tex <==
\begin{tabular}{llllllllll}
\toprule
    &                             & \multicolumn{4}{c}{AmbigDocs}                                                                                                                                                     & \multicolumn{4}{c}{WebTrack09-12}                                                                                                                          \\ \cmidrule(lr){3-6} \cmidrule(lr){7-10}
\multirow{2}{*}{LLM}     & \multirow{2}{*}{Expansion}  & \multicolumn{2}{c}{NDCG@10}                                                             & \multicolumn{2}{c}{Recall@100}                                                          & \multicolumn{2}{c}{NDCG@10}                                                             & \multicolumn{2}{c}{Recall@100}                                             \\ \cmidrule{3-10} 
    &                             & \multicolumn{1}{c}{high}   & \multicolumn{1}{c}{low}                          & \multicolumn{1}{c}{high}   & \multicolumn{1}{c}{low}                          & \multicolumn{1}{c}{high}    & \multicolumn{1}{c}{low}                      & \multicolumn{1}{c}{high}    & \multicolumn{1}{c}{low}     \\ \midrule \midrule
\multirow{4}{*}{GPT}     & \multicolumn{1}{l|}{No Exp} & 19.70 & \multicolumn{1}{l|}{35.55}      & 60.01 & \multicolumn{1}{l|}{76.94}      & 44.06  & \multicolumn{1}{l|}{45.42}  & 58.78  & 64.70      \\
    & \multicolumn{1}{l|}{Q2E}    & +1.94 & \multicolumn{1}{l|}{\bf{+3.70}} & +0.58 & \multicolumn{1}{l|}{\bf{+1.87}} & +14.64 & \multicolumn{1}{l|}{+11.60} & -7.67  & \bf{+0.11} \\
    & \multicolumn{1}{l|}{Q2D}    & +3.11 & \multicolumn{1}{l|}{\bf{+4.72}} & +2.03 & \multicolumn{1}{l|}{+3.01}      & +14.27 & \multicolumn{1}{l|}{+17.82} & -12.93 & \bf{-4.45} \\
    & \multicolumn{1}{l|}{GaQR (T)}   & +2.78 & \multicolumn{1}{l|}{\bf{+4.34}} & +4.11 & \multicolumn{1}{l|}{+4.35}      & +12.01 & \multicolumn{1}{l|}{+10.26} & -4.64  & \bf{+2.87} \\ \cline{1-2}
\multirow{3}{*}{Llama8b}   & \multicolumn{1}{l|}{Q2E}    & +1.09 & \multicolumn{1}{l|}{\bf{+2.44}} & -0.49 & \multicolumn{1}{l|}{\bf{+0.86}} & +11.31 & \multicolumn{1}{l|}{+5.08}  & -17.39 & \bf{-4.60} \\
    & \multicolumn{1}{l|}{Q2D}    & +2.61 & \multicolumn{1}{l|}{\bf{+4.19}} & -0.02 & \multicolumn{1}{l|}{\bf{+1.78}} & +13.58 & \multicolumn{1}{l|}{+13.54} & -13.90 & \bf{-5.37} \\
    & \multicolumn{1}{l|}{GaQR (S)}   & +2.31 & \multicolumn{1}{l|}{\bf{+3.69}} & +3.58 & \multicolumn{1}{l|}{+3.83}      & +12.45 & \multicolumn{1}{l|}{+10.97} & -11.09 & -5.93      \\ \bottomrule
\end{tabular}

==> tables/rq2_table.tex <==
\begin{tabular}{lllcccccc}
    \hline
                                                    &                                             &                           & \multicolumn{2}{c}{AmbigDocs}                                                               & \multicolumn{2}{c}{web09}                                                                   & \multicolumn{2}{c}{AmbigQA}                                           \\ \cline{4-9} 
Retrieval                                        & LLM                                         & Expansion                 & NDCG@10                            & Recall@100                                             & NDCG@10                           & Recall@100                                              & NDCG@10                           & Recall@100                        \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{BM25}}       & \multicolumn{1}{l|}{\multirow{3}{*}{GPT}}   & \multicolumn{1}{l|}{Q2E}  & \cellcolor[HTML]{FED2D1}\bf{1.76}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FEDADA}\bf{1.29}} & \cellcolor[HTML]{D1D2F7}-3.04     & \multicolumn{1}{c|}{\cellcolor[HTML]{FD807C}\bf{7.78}}  & \cellcolor[HTML]{F6F6FD}-0.28     & \cellcolor[HTML]{FEF0F0}0.34      \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Q2D}  & \cellcolor[HTML]{FED4D3}\bf{1.61}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FEE1E0}0.98}      & \cellcolor[HTML]{FEB5B3}3.55      & \multicolumn{1}{c|}{\cellcolor[HTML]{FD7874}\bf{8.48}}  & \cellcolor[HTML]{FEC3C1}\bf{2.65} & \cellcolor[HTML]{FDA7A5}\bf{4.55} \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{GaQR} & \cellcolor[HTML]{FED5D4}\bf{1.56}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF3F3}0.24}      & \cellcolor[HTML]{E0E0F9}-1.75     & \multicolumn{1}{c|}{\cellcolor[HTML]{FD8380}\bf{7.51}}  & \cellcolor[HTML]{FEF0EF}0.36      & \cellcolor[HTML]{FEE0DF}1.02      \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{BM25}}       & \multicolumn{1}{l|}{\multirow{3}{*}{L-8b}} & \multicolumn{1}{l|}{Q2E}  & \cellcolor[HTML]{FED9D8}\bf{1.35}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FED9D8}\bf{1.35}} & \cellcolor[HTML]{B3B5F2}-6.23     & \multicolumn{1}{c|}{\cellcolor[HTML]{FD6864}\bf{12.79}} & \cellcolor[HTML]{F6F6FD}-0.29     & \cellcolor[HTML]{FECFCE}1.92      \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Q2D}  & \cellcolor[HTML]{FED5D4}\bf{1.58}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FED1D0}\bf{1.80}} & \cellcolor[HTML]{FCFCFE}-0.04     & \multicolumn{1}{c|}{\cellcolor[HTML]{FD7774}\bf{8.53}}  & \cellcolor[HTML]{EEEFFC}-0.69     & \cellcolor[HTML]{FEB6B4}\bf{3.50} \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{GaQR} & \cellcolor[HTML]{FED9D8}\bf{1.38}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FEF3F3}0.25}      & \cellcolor[HTML]{E3E3FA}-1.48     & \multicolumn{1}{c|}{\cellcolor[HTML]{FD9F9D}5.16}       & \cellcolor[HTML]{ECECFB}-0.84     & \cellcolor[HTML]{ECEDFB}-0.81     \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{ANCE}}       & \multicolumn{1}{l|}{\multirow{3}{*}{L-8b}} & \multicolumn{1}{l|}{Q2E}  & \cellcolor[HTML]{DDDEF9}\bf{-1.93} & \multicolumn{1}{c|}{\cellcolor[HTML]{FEDFDE}1.05}      & \cellcolor[HTML]{FEBEBD}2.94      & \multicolumn{1}{c|}{\cellcolor[HTML]{FD8D8A}\bf{6.63}}  & \cellcolor[HTML]{FEC6C5}\bf{2.43} & \cellcolor[HTML]{FED8D7}1.42      \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Q2D}  & \cellcolor[HTML]{F1F1FC}-0.53      & \multicolumn{1}{c|}{\cellcolor[HTML]{FEC4C3}\bf{2.56}} & \cellcolor[HTML]{FD9391}6.12      & \multicolumn{1}{c|}{\cellcolor[HTML]{FEC6C5}2.44}       & \cellcolor[HTML]{FEBFBE}\bf{2.87} & \cellcolor[HTML]{FEEFEE}0.40      \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{GaQR} & \cellcolor[HTML]{E8E9FB}-1.10      & \multicolumn{1}{c|}{\cellcolor[HTML]{FED3D2}\bf{1.70}} & \cellcolor[HTML]{FD7C78}8.14      & \multicolumn{1}{c|}{\cellcolor[HTML]{FDB0AD}3.96}       & \cellcolor[HTML]{FEDDDC}1.17      & \cellcolor[HTML]{FEF5F5}0.19      \\ \hline 
\multicolumn{1}{l|}{\multirow{3}{*}{Contriever}} & \multicolumn{1}{l|}{\multirow{3}{*}{L-8b}} & \multicolumn{1}{l|}{Q2E}  & \cellcolor[HTML]{E9E9FB}-1.07      & \multicolumn{1}{c|}{\cellcolor[HTML]{FD7874}\bf{8.48}} & \cellcolor[HTML]{FEC4C2}2.60      & \multicolumn{1}{c|}{\cellcolor[HTML]{FD706C}\bf{9.19}}  & \cellcolor[HTML]{FEECEB}0.51      & \cellcolor[HTML]{FED1D0}1.79      \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Q2D}  & \cellcolor[HTML]{CECFF6}\bf{-3.32} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD7874}\bf{8.52}} & \cellcolor[HTML]{FDAAA7}4.39      & \multicolumn{1}{c|}{\cellcolor[HTML]{FDAFAD}4.00}       & \cellcolor[HTML]{EFF0FC}-0.63     & \cellcolor[HTML]{FEE1E1}0.95      \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{GaQR} & \cellcolor[HTML]{E6E7FA}\bf{-1.24} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD8784}\bf{7.16}} & \cellcolor[HTML]{FDB2B0}3.81      & \multicolumn{1}{c|}{\cellcolor[HTML]{FD8B88}\bf{6.84}}  & \cellcolor[HTML]{EDEDFB}-0.80     & \cellcolor[HTML]{FEE3E2}0.87      \\ \hline 
\multicolumn{1}{l|}{\multirow{3}{*}{E5-base-v2}} & \multicolumn{1}{l|}{\multirow{3}{*}{L-8b}} & \multicolumn{1}{l|}{Q2E}  & \cellcolor[HTML]{A5A6EF}\bf{-8.01} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD9C99}\bf{5.44}} & \cellcolor[HTML]{FDA7A4}4.60      & \multicolumn{1}{c|}{\cellcolor[HTML]{FD6864}\bf{11.41}} & \cellcolor[HTML]{FEB5B3}\bf{3.59} & \cellcolor[HTML]{FDB2AF}\bf{3.82} \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Q2D}  & \cellcolor[HTML]{AFB1F1}\bf{-6.68} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD9895}\bf{5.74}} & \cellcolor[HTML]{FD9895}\bf{5.74} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD9C99}\bf{5.45}}  & \cellcolor[HTML]{FEEDEC}0.47      & \cellcolor[HTML]{FECECD}1.95      \\
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{GaQR} & \cellcolor[HTML]{9FA1EE}\bf{-8.69} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD9C9A}\bf{5.40}} & \cellcolor[HTML]{FD7572}\bf{8.72} & \multicolumn{1}{c|}{\cellcolor[HTML]{FD8480}\bf{7.44}}  & \cellcolor[HTML]{FECDCC}2.04      & \cellcolor[HTML]{FEB3B1}\bf{3.69} \\ \hline
\end{tabular}
